FIC-TSC: Learning Time Series Classification with Fisher Information Constraint

Analyzing time series data is crucial to a wide spectrum of applications, including economics, online marketplaces, and human healthcare. In particular, time series classification plays an indispensable role in segmenting different phases in stock markets, predicting customer behavior, and classifying worker actions and engagement levels. These aspects contribute significantly to the advancement of automated decision-making and system optimization in real-world applications. However, there is a large consensus that time series data often suffers from domain shifts between training and test sets, which dramatically degrades the classification performance. Despite the success of (reversible) instance normalization in handling the domain shifts for time series regression tasks, its performance in classification is unsatisfactory. In this paper, we propose \textit{FIC-TSC}, a training framework for time series classification that leverages Fisher information as the constraint. We theoretically and empirically show this is an efficient and effective solution to guide the model converge toward flatter minima, which enhances its generalizability to distribution shifts. We rigorously evaluate our method on 30 UEA multivariate and 85 UCR univariate datasets. Our empirical results demonstrate the superiority of the proposed method over 14 recent state-of-the-art methods.

==> table_original.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{table*}[!t]
\centering
\caption{Comparison of classification accuracy by our method with recent alternative methods for multivariate time series classification (26 UEA datasets). We highlight the best results in \textcolor{red}{\textbf{bold}} and the second-best results with  \textcolor{blue}{\underline{underlining}}.
\textit{Uni.} indicates we set the consistent hyperparameters for all datasets, while \textit{Full} indicates we perform dataset-wise grid search for hyperparameters. To ensure the robustness and rigor of our approach, we included \textit{Full} at the end but did not participate in the comparison. The accuracy is averaged over 5 runs. }
\label{tab:result1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|
>{\columncolor[HTML]{EFEFEF}}c ccccccccccc|c}\toprule
\multicolumn{1}{c}{\textbf{Dataset}} & \textbf{\begin{tabular}[c]{@{}c@{}}Ours\\    (Uni.)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}MILLET\\      ICLR'24\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TodyNet\\      Inf. Sci.'24\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ConvTran\\      ECML'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}ROCKET\\      ECML'20\end{tabular}}  & \textbf{\begin{tabular}[c]{@{}c@{}}TsLaNet\\      ICML'24\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}GPT4TS\\      NeurIPS'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TimesNet\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}CrossFormer\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}PatchTST\\      ICLR'23\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}TS-TCC\\      IJCAI'21\end{tabular}} & \textbf{Linear} & {\color[HTML]{455266} \textbf{\begin{tabular}[c]{@{}c@{}}Ours\\ (Full)\end{tabular}}} \\ \midrule
ArticularyWordRecognition & {\color[HTML]{FF0000} \textbf{99.3}} & 99.0 & 98.2 & 98.3 & {\color[HTML]{FF0000} \textbf{99.3}} & 99.0 & 93.3 & 96.2 & 98.0 & 97.7 & 98.0 & 93.1 & {\color[HTML]{455266} 99.8} \\
AtrialFibrillation & {\color[HTML]{FF0000} \textbf{56.7}} & 43.3 & 46.7 & 40.0 & 20.0 & 40.0 & 33.3 & 33.3 & 46.7 & {\color[HTML]{0000FF} {\ul 53.3}} & 33.3 & 46.7 & {\color[HTML]{455266} 60.0} \\
BasicMotions & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{FF0000} \textbf{100.0}} & 92.5 & {\color[HTML]{FF0000} \textbf{100.0}} & 90.0 & 92.5 & {\color[HTML]{FF0000} \textbf{100.0}} & 85.0 & {\color[HTML]{455266} 100.0} \\
Cricket & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{FF0000} \textbf{100.0}} & 98.6 & {\color[HTML]{FF0000} \textbf{100.0}} & 98.6 & 98.6 & 8.3 & 87.5 & 84.7 & 84.7 & 93.1 & 91.7 & {\color[HTML]{455266} 100.0} \\
Epilepsy & {\color[HTML]{FF0000} \textbf{98.9}} & {\color[HTML]{0000FF} {\ul 98.6}} & 96.4 & 98.6 & 98.6 & 98.6 & 85.5 & 78.1 & 73.2 & 65.9 & 97.1 & 60.1 & {\color[HTML]{455266} 100.0} \\
EthanolConcentration & 39.2 & 32.3 & {\color[HTML]{0000FF} {\ul 42.4}} & 36.1 & {\color[HTML]{FF0000} 42.6} & 30.4 & 25.5 & 27.7 & 35.0 & 28.9 & 32.3 & 33.5 & {\color[HTML]{455266} 40.1} \\
FaceDetection & 68.4 & {\color[HTML]{FF0000} \textbf{69.2}} & 67.7 & 67.2 & 64.7 & 66.8 & 65.6 & 67.5 & 66.2 & {\color[HTML]{0000FF} {\ul 69.0}} & 63.1 & 67.4 & {\color[HTML]{455266} 69.2} \\
FingerMovements & {\color[HTML]{FF0000} \textbf{65.0}} & {\color[HTML]{0000FF} {\ul 64.0}} & 62.5 & 56.0 & 61.0 & 61.0 & 57.0 & 59.4 & {\color[HTML]{0000FF} {\ul 64.0}} & 62.0 & 44.0 & {\color[HTML]{0000FF} {\ul 64.0}} & {\color[HTML]{455266} 71.5} \\
HandMovementDirection & 49.3 & 50.7 & 54.1 & 40.5 & 50.0 & 52.7 & 18.9 & 50.0 & {\color[HTML]{0000FF} {\ul 58.1}} & {\color[HTML]{0000FF} {\ul 58.1}} & {\color[HTML]{FF0000} \textbf{64.9}} & {\color[HTML]{0000FF} {\ul 58.1}} & {\color[HTML]{455266} 54.7} \\
Handwriting & {\color[HTML]{0000FF} {\ul 61.6}} & {\color[HTML]{FF0000} \textbf{69.8}} & 47.9 & 37.5 & 48.5 & 57.9 & 3.8 & 26.2 & 26.2 & 26.0 & 47.8 & 22.5 & {\color[HTML]{455266} 73.0} \\
Heartbeat & {\color[HTML]{FF0000} \textbf{81.0}} & 76.8 & {\color[HTML]{0000FF} {\ul 79.0}} & 78.5 & 69.8 & 77.6 & 36.6 & 74.5 & 76.6 & 76.6 & 77.1 & 73.2 & {\color[HTML]{455266} 82.0} \\
InsectWingbeat & 71.1 & {\color[HTML]{FF0000} \textbf{72.0}} & 63.0 & {\color[HTML]{0000FF} {\ul 71.3}} & 41.8 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & 10.0 & {\color[HTML]{455266} 72.3} \\
Japanese Vowels & 99.1 & {\color[HTML]{FF0000} \textbf{99.6}} & 97.6 & 98.9 & 95.7 & {\color[HTML]{0000FF} {\ul 99.2}} & 98.1 & 97.8 & 98.9 & 98.7 & 97.3 & 97.8 & {\color[HTML]{455266} 99.6} \\
Libras & 79.4 & 91.1 & 84.4 & {\color[HTML]{0000FF} {\ul 92.8}} & 83.9 & {\color[HTML]{FF0000} \textbf{92.8}} & 79.4 & 77.8 & 76.1 & 81.1 & 86.7 & 73.3 & {\color[HTML]{455266} 91.7} \\
LSST & 65.3 & 50.2 & 65.1 & 61.6 & 54.1 & {\color[HTML]{0000FF} {\ul 66.3}} & 46.4 & 59.2 & 42.8 & {\color[HTML]{FF0000} \textbf{67.8}} & 49.2 & 35.8 & {\color[HTML]{455266} 66.8} \\
MotorImagery & {\color[HTML]{FF0000} \textbf{65.0}} & 61.5 & {\color[HTML]{0000FF} {\ul 64.0}} & 56.0 & 53.0 & 62.0 & 50.0 & 51.0 & 61.0 & 61.0 & 47.0 & 61.0 & {\color[HTML]{455266} 68.5} \\
NATOPS & {\color[HTML]{FF0000} \textbf{98.9}} & {\color[HTML]{0000FF} {\ul 98.3}} & 95.6 & 94.4 & 83.3 & 95.6 & 91.7 & 81.8 & 88.3 & 96.7 & 96.1 & 93.9 & {\color[HTML]{455266} 99.2} \\
PEMS-SF & 79.2 & 63.0 & {\color[HTML]{FF0000} \textbf{96.1}} & 82.8 & 75.1 & 83.8 & 87.3 & 88.1 & 82.1 & {\color[HTML]{0000FF} {\ul 88.4}} & 86.7 & 82.1 & {\color[HTML]{455266} 87.9} \\
PenDigits & 97.6 & 92.6 & 98.7 & 98.7 & 97.3 & {\color[HTML]{0000FF} {\ul 98.9}} & 97.7 & 98.2 & 93.7 & {\color[HTML]{FF0000} \textbf{99.2}} & 98.5 & 92.9 & {\color[HTML]{455266} 98.5} \\
PhonemeSpectra & {\color[HTML]{0000FF} {\ul 31.3}} & {\color[HTML]{FF0000} \textbf{34.3}} & 31.2 & 30.6 & 17.6 & 17.8 & 3.0 & 18.2 & 7.6 & 11.7 & 25.9 & 7.1 & {\color[HTML]{455266} 32.3} \\
RacketSports & {\color[HTML]{0000FF} {\ul 89.8}} & 88.2 & 84.5 & 86.2 & 86.2 & {\color[HTML]{FF0000} \textbf{90.8}} & 77.0 & 82.6 & 81.6 & 84.2 & 84.9 & 79.0 & {\color[HTML]{455266} 90.8} \\
SelfRegulationSCP1 & 90.1 & 88.1 & 90.4 & 91.8 & 84.6 & {\color[HTML]{0000FF} {\ul 91.8}} & 91.5 & 77.4 & {\color[HTML]{FF0000} 92.5} & 89.8 & 91.1 & 88.4 & {\color[HTML]{455266} 90.3} \\
SelfRegulationSCP2 & 59.4 & {\color[HTML]{0000FF} {\ul 59.4}} & 59.4 & 58.3 & 54.4 & {\color[HTML]{FF0000} \textbf{61.7}} & 51.7 & 52.8 & 53.3 & 54.4 & 53.9 & 51.7 & {\color[HTML]{455266} 60.8} \\
SpokenArabicDigits & {\color[HTML]{FF0000} \textbf{100.0}} & {\color[HTML]{0000FF} {\ul 99.9}} & 99.1 & 99.5 & 99.2 & 99.9 & 99.4 & 98.4 & 96.4 & 99.7 & 99.8 & 96.7 & {\color[HTML]{455266} 100.0} \\
StandWalkJump & {\color[HTML]{FF0000} \textbf{63.3}} & 53.3 & 36.7 & 33.3 & 46.7 & 46.7 & 33.3 & 53.3 & 53.3 & {\color[HTML]{0000FF} {\ul 60.0}} & 40.0 & {\color[HTML]{0000FF} {\ul 60.0}} & {\color[HTML]{455266} 66.7} \\
UWaveGestureLibrary & 90.2 & 90.8 & 86.3 & 89.1 & {\color[HTML]{FF0000} \textbf{94.4}} & {\color[HTML]{0000FF} {\ul 91.3}} & 84.4 & 83.1 & 81.6 & 80.0 & 86.3 & 81.9 & {\color[HTML]{455266} 93.0} \\ \midrule
\textbf{Avg.} & {\color[HTML]{FF0000} \textbf{76.9}} & {\color[HTML]{0000FF} \ul {74.8}} & {\color[HTML]{0000FF} \ul {74.8}} & 73.0 & 70.0 & 72.7 & 58.5 & 66.6 & 66.8 & 69.1 & 69.4 & 65.6 & {\color[HTML]{455266} 79.6} \\ \bottomrule
\end{tabular}%
}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

